Garment Recovery with Shape and Deformation Priors

While modeling people wearing tight-fitting clothing has made great strides in recent years, loose-fitting clothing remains a challenge. We propose a method that delivers realistic garment models from real-world images, regardless of garment shape or deformation. To this end, we introduce a fitting approach that utilizes shape and deformation priors learned from synthetic data to accurately capture garment shapes and deformations, including large ones. Not only does our approach recover the garment geometry accurately, it also yields models that can be directly used by downstream applications such as animation and simulation.

==> figs/cut_opening.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/cut_opening_p.pdf}
    %\vspace{-0.3cm}
    \caption{\textbf{The cutting and flattening for open shirt.} (a) The original mesh. (b) The cut surfaces. (c) The flattened panels.}
    \label{fig:cut_opening}
    %\vspace{-0.45cm}
\end{figure}


==> figs/cut_skirt.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/cut_skirt_p.pdf}
    %\vspace{-0.3cm}
    \caption{\textbf{The cutting and flattening for skirt.} (a) The original mesh. (b) The cut surfaces. (c) The flattened panels.}
    \label{fig:cut_skirt}
    %\vspace{-0.45cm}
\end{figure}


==> figs/cut_trousers.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/cut_trousers_p.pdf}
    %\vspace{-0.3cm}
    \caption{\textbf{The cutting and flattening for trousers.} (a) The original mesh. (b) The cut surfaces. (c) The flattened panels.}
    \label{fig:cut_trousers}
    %\vspace{-0.45cm}
\end{figure}


==> figs/econ.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.87\textwidth]{figs/econ_p.pdf}
    %\vspace{-0.3cm}
    \caption{\textbf{Comparison with ECON~\cite{Xiu23}.} Our method can recover realistic separated open surfaces for garments, while ECON generates closed meshes that encompass both the garments and the body.}
    \label{fig:econ}
    %\vspace{-0.45cm}
\end{figure*}


==> figs/fail.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/fail_p.pdf}
    %\vspace{-0.3cm}
    \caption{(a) The self-interpenetration of the estimated SMPL body leads to (b) the intersection between the reconstructed skirt and the hand of the body.}
    \label{fig:fail}
    %\vspace{-0.45cm}
\end{figure}


==> figs/fail2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/fail2_p.pdf}
    %\vspace{-0.3cm}
    \caption{(a) The inaccurate normal estimation of the skirt leads to (b) the artifacts on the reconstructed surface.}
    \label{fig:fail2}
    %\vspace{-0.45cm}
\end{figure}


==> figs/grade.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/grade_p.pdf}
    %\vspace{-0.3cm}
    \caption{\textbf{Transfer to the neutral body.} (a) The original shirt on $\beta$-shape body. (b) The shirt transferred by Eq. \ref{eq:diffuse} on the neural body. (c) The shirt refined by Eq. \ref{eq:grade}.}
    \label{fig:grade}
    %\vspace{-0.45cm}
\end{figure*}


==> figs/occupancy2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/occupancy2_p.pdf}
    %\vspace{-0.3cm}
    \caption{(a) The input image (top) and the corresponding rest mesh recovered by ISP (bottom). (b) The occupancy maps predicted by the deformation model $\mathcal{D}$. (c) The occupancy maps recovered by the optimization of the latent code of ISP (Eq. \ref{eq:z}).}
    \label{fig:occupancy}
    %\vspace{-0.45cm}
\end{figure}

==> figs/simulation.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/simulation_p.pdf}
    %\vspace{-0.3cm}
    \caption{\textbf{Simulation.} }
    \label{fig:simulation}
    %\vspace{-0.45cm}
\end{figure}

